PANDORA: Polarization-Aided Neural Decomposition Of Radiance

Reconstructing an object's geometry and appearance from multiple images, also known as inverse rendering, is a fundamental problem in computer graphics and vision. Inverse rendering is inherently ill-posed because the captured image is an intricate function of unknown lighting conditions, material properties and scene geometry. Recent progress in representing scene properties as coordinate-based neural networks have facilitated neural inverse rendering resulting in impressive geometry reconstruction and novel-view synthesis. Our key insight is that polarization is a useful cue for neural inverse rendering as polarization strongly depends on surface normals and is distinct for diffuse and specular reflectance. With the advent of commodity, on-chip, polarization sensors, capturing polarization has become practical. Thus, we propose PANDORA, a polarimetric inverse rendering approach based on implicit neural representations. From multi-view polarization images of an object, PANDORA jointly extracts the object's 3D geometry, separates the outgoing radiance into diffuse and specular and estimates the illumination incident on the object. We show that PANDORA outperforms state-of-the-art radiance decomposition techniques. PANDORA outputs clean surface reconstructions free from texture artefacts, models strong specularities accurately and estimates illumination under practical unstructured scenarios.

==> 03_old_neural_radiance.tex <==
\subsection{Notations}
We aim to recover the object shape, material properties and illumination from multi-view images. We assume the camera poses are already obtained, for example, using COLMAP. Thus for any pixel in the captured images, the camera position $\mathbf{o}$ and camera ray direction $\mathbf{d}$ are known. Consider that this ray hits the object's surface at position $x$. The object's surface normals, diffuse albedo and roughness are denoted as $\mathbf{n}$, $\rho$ and $\alpha$ respectively.
\subsection{Image formation by volume rendering}
To render the radiance measured by camera ray given by $\mathbf{o}$ and $\mathbf{d}$, the ray is sampled at $\mathcal{T}$ points. For a sample on the ray with travel distance $t$, its location is denoted at $\mathbf{r}(t) = \mathbf{o}+t\mathbf{d}$. The radiance contribution of this sample depends on the scene opacity, $\sigma(\mathbf{r}(t))$ and outgoing radiance $L_o(\mathbf{r}(t),\mathbf{d})$. The observed radiance, $L(\mathbf{o},\mathbf{d})$ is denoted by the integral, 
\begin{align}
    L_o(\mathbf{o},\mathbf{d}) = \int_{0}^{\infty}{T(t)\sigma(\mathbf{r}(t))L_o(\mathbf{r}(t),\mathbf{d})} dt \;,
    \label{eq:vol_render_int}
\end{align}
where $T(t) = exp\left(-\int_{0}^{\infty}{\sigma(\mathbf{r}(t))}\right)$ is the probablity that the ray travels to $t$ without getting occluded.
\subsection{Neural Radiance Fields (NeRFs)}
NeRF \cite{mildenhall2020} models the opacity $\sigma$ and outgoing radiance $L_o$ using coordinate-based MLPs with sinusoidal positional encodings. These MLPs are trained to minimize the loss between net radiance rendered using the volumetric model in Eq. \ref{eq:vol_render_int} and the captured radiance.

In reality, the camera ray intersects the surface at only a single point. If the intersection occurs for the point on ray $t^*$ then the ideal value of scene opacity $\sigma(\mathbf{r}(t))$ is $0$ for $t<t^*$ and $1$ for $t>t^*$. Due to this sharp discontinuity, modelling opacity is challenging in the volume rendering frame work and requires efficient strategies to sample points on the ray. 
\subsection{Incorporating surface rendering in NeRFs}
VolSDF \cite{yariv2021volume} demonstrate reconstruction quality improves when the coordinate-based networks are used to model the object's signed distance field (SDF) $d$ instead of the scene opacity. The opacity is estimated from $d$ as
\begin{align}
    \sigma(x) = \alpha \Psi_{\beta}(-d(x)) \;,
\end{align}
where $\alpha$,$\beta$ are learnable parameters and $\Psi$ is the Cumulative Distribution Function of the Laplace distribution with zero mean and scale $\beta$.
Another advantage of modelling SDF is the the surface normals are analytically modelled as the spatial gradient of the SDF, 
\begin{align}
    \mathbf{n}(x) = \nabla_x(d(x)) \;.
\end{align}
NeRF and VolSDF directly model the outgoing radiance which is a combination of the object's reflectance and illumination. Thus, it's not possible to use the model for separating diffuse and specular reflectance or for re-lighting the object under a different lighting. 

\subsection{Extending NeRFs for radiance decomposition}
The outgoing radiance depends on the surface reflectance parameters $\rho$ and $\alpha$ along with the incident illumination $L_i$. Using rendering equation and the Cook-Torrance reflectance model, the outgoing radiance can be written as a combination of diffuse and specular components.
\begin{align}
    L_o(\mathbf{x},\omega_o) &= L_d(\mathbf{x}) + L_s(\mathbf{x},\omega_o) \;,\\
    L_s(\mathbf{x},\omega_o) &= \int_{\Omega}{L_i(\mathbf{x},\omega_i) f_s(\mathbf{x},\omega_i,\omega_o,\mathbf{n},\alpha) d\omega_i} \;.
\end{align}
We model the specular BRDF $f_s$ using microfacet model where $f_s$ depends on the half-angle $\omega_h =(\omega_i+\omega_o)/2$ as,
\begin{align}
    f_s = \frac{F(\omega_i,\mathbf{n}),D(\omega_h,\mathbf{n},\alpha)G(\omega_i,\omega_o,\alpha)}{4cos(\omega_i)cos(\omega_o)} \;,
\end{align}
where D is GGX distribution, G is Smith's shadowing/masking function and F is Fresnel reflectance.
Integration along the incident angles is computational intractable 
and decomposition of $L_d$,$\alpha$ and $L_i$ from $L_o$ is inherently ill-posed. Several approaches have been proposed towards overcoming these limitations. NeRFactor \cite{zhang2021nerfactor} proposes modelling BRDF as data-driven embeddings learned using MeRL BRDF dataset. NeuralPIL \cite{boss2021neural} propose pre-integrating the lighting using a pre-trained neural network along with learning embeddings for the BRDF and illumination. Ref-NeRF \cite{verbin2021ref} introduce integrated directional embeddings for modelling the illumination integration as a function of the roughness. We found the IDE approach proposed by Verbin et al. was the most effective in modeling surface roughness. The IDE mapped the input direction ($\omega_i$) and roughness factor ($\alpha$) to a set of embeddings using the spherical harmonics:

\begin{align}
IDE(\omega_i, \alpha, L)=\\ 
\{ \exp(-\alpha \ell(\ell+1)/2) \mathbf{Y}^\ell _m(\omega_i) \mid m\in[-\ell,\ell], \ell\in\{ 1,2,...2^L\}\}
\end{align}

While these approaches provide promising decomposition in simple scenarios, they suffer from artifacts (Figure \ref{fig:sim_radiance}). Our claim is that incorporating polarimetric cues improves radiance decomposition compared to existing intensity-based approaches.


==> figs_tex/baseline_features_table.tex <==
\begin{table}[!h]
    \centering
    \small
    % \setlength{\tabcolsep}{4 pt}
    \begin{tabular}{|lMLLL|}
        \hline
        \rowcolor{black}
        \textcolor{white}{Approach} & 
        \textcolor{white}{Surface estimation quality} & 
        \textcolor{white}{Can separate diffuse and specular ?} &
        \textcolor{white}{Can separate lighting and reflectance ?} &
        \textcolor{white}{Can exploit polarimetric cues ?}\\
        \hline
        NeRF &
        \cellcolor{red!15}{Low} &
        No &
        No &
        No \\
        \hline
        VolSDF &
        High &
        No &
        No &
        No \\
        \hline
        NeuralPIL &
        Med &
        Yes &
        Yes &
        No \\
        \hline
        {RefNeRF} &
        High &
        Yes &
        No &
        No \\
        \hline 
        \textbf{PANDORA} &
        High &
        Yes &
        Yes &
        Yes \\
        \hline 
    \end{tabular}
    \caption{\textbf{Key features of existing neural inverse rendering techniques}}
    \label{tab:baseline_features}
\end{table}

==> figs_tex/effect_of_roughness.tex <==
\begin{figure*}
\begin{center}
   \includegraphics[width=1.0\linewidth]{figs_png/roughness_v1.png}
\end{center}
  \caption{\textit{Surface roughness estimation.} Our method is able to estimate the surface roughness parameter, $\alpha$ (center). We can also estimate the corresponding environment map without surface roughness (left).}
  \label{fig:roughness_estimation}
\end{figure*}

==> figs_tex/older_figs.tex <==
% PANDORA can be used for both radiance decomposition, but also novel-view synthesis on the separated diffuse and specular components \ref{fig:novel_view_diff_spec}.

% \begin{figure}[ht!]
% \begin{center}
%   \includegraphics[width=1.0\linewidth]{figs/figXX_novel_view_diff_spec.png}
% \end{center}
%   \caption{\textit{Our method can be used for novel view synthesis as well as radiance decomposition.} Using a set of training images (top row) that contain both diffuse and specular reflection, our method can perform not only radiance decomposition but also novel view synthesis of the separated diffuse and specular components (middle row). Detailed features of these components are shown in the bottom row.}
%   \label{fig:novel_view_diff_spec}
% \end{figure}
% \begin{figure}[ht!]
% \begin{center}
%   \includegraphics[width=1.0\linewidth]{figs/polarized_diff_spec_sep.png}
% \end{center}
% \caption{\textit{PANDORA achieves superior radiance decomposition compared to traditional methods.} We test PANDORA against traditional neural implicit representations (NeRF, VolSDF). While other algorithms fail to achieve good separation of diffuse-specular components, our approach can resolve even detailed features in the specular reflection.}
% \label{fig:diff_spec_sep}

% \end{figure}

% \begin{figure}
% \begin{center}
%   \includegraphics[width=1.0\linewidth]{figs/figXX_learned_env_map.png}
% \end{center}
% \caption{\textit{Our method can also be used to estimate the environment map.} We use an MLP to estimate the specular reflection from the target object. This MLP can also be used to estimate the environment map, as shown above. The blue and red inset features show the detailed features, which are learned by the network. We compare the quality of the estimated environment map with (bottom) and without (middle) polarization information.}
% \label{fig:env_map}
% \end{figure}

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/initial_comparison.png}
%     \caption{\textit{Initial comparisons with baseline}}
%     \label{fig:my_label}
% \end{figure}

==> figs_tex/real_params.tex <==
\begin{figure*}
\centering
\setlength{\tabcolsep}{0pt}
\begin{tabular}{rccc@{\hskip 3pt}|@{\hskip 3pt}ccc}
 & Albedo & Roughness & Illumination
 & Albedo & Roughness & Illumination
\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\rotatebox[origin=c]{90}{NeuralPIL}&
\raisebox{-0.5\height}{\igr{0.12}{5cm}{3.25cm}{6cm}{0.25cm}
{out_imgs/test_imgs_400001_Our_gnome/0_fine_diffuse.png}}&
\raisebox{-0.5\height}{\igr{0.12}{5cm}{3.25cm}{6cm}{0.25cm}
{out_imgs/test_imgs_400001_Our_gnome/0_fine_roughness.png}}&
\raisebox{-0.5\height}{\igr{0.26}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/test_imgs_400001_Our_gnome/0_fine_env_map.png}}&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\raisebox{-0.5\height}{\igr{0.12}{4cm}{2cm}{7.cm}{1.5cm}
{out_imgs/test_imgs_386880_Our_black_vase_v2/0_fine_diffuse.png}}&
\raisebox{-0.5\height}{\igr{0.12}{4cm}{2cm}{7.cm}{1.5cm}
{out_imgs/test_imgs_386880_Our_black_vase_v2/0_fine_roughness.png}}&
\raisebox{-0.5\height}{\igr{0.26}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/test_imgs_386880_Our_black_vase_v2/0_fine_env_map.png}}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox[origin=c]{90}{Ours}&
\raisebox{-0.5\height}{\igr{0.12}{5cm}{3.25cm}{6cm}{0.25cm}
{out_imgs/294_test_018_v00_imgs/pred_000_alb.png}}&
\raisebox{-0.5\height}{\igr{0.12}{5cm}{3.25cm}{6cm}{0.25cm}
{out_imgs/294_test_018_v00_imgs/pred_000_rough.png}}&
\raisebox{-0.5\height}{\igr{0.26}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/294_test_018_v00_imgs/env_map_alpha=0.03.png}}&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\raisebox{-0.5\height}{\igr{0.12}{4.cm}{2cm}{7.5cm}{1.5cm}
{out_imgs/295_test_020_v00_imgs/pred_000_alb.png}}&
\raisebox{-0.5\height}{\igr{0.12}{4.cm}{2cm}{7.5cm}{1.5cm}
{out_imgs/295_test_020_v00_imgs/pred_000_rough.png}}&
\raisebox{-0.5\height}{\igr{0.26}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/295_test_020_v00_imgs/env_map_alpha=0.03.png}}
\\

\end{tabular}
\caption{\textbf{Reflectance parameters and illumination on real dataset}}
\end{figure*}

==> figs_tex/sim_illum.tex <==
\begin{figure}
\centering
\setlength{\tabcolsep}{0pt}
\begin{tabular}{cc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
NeuralPIL on unknown object & NeuralPIL on known object\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_neuralpil/0_fine_env_map.png}}&
\raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/gt_env_maps/christmas_neuralpil_paper.jpg}}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ours on unknown object & Ground Truth \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_ours/env_map_alpha=0.03.png}}&
\raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/gt_env_maps/christmas.jpg}}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \multicolumn{2}{c}{
% \raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
% {out_imgs/gt_env_maps/20060807_wells6_hd.png}}}
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \rotatebox[origin=c]{90}{Train Views}&
% \raisebox{-0.5\height}{\igr{0.12}{1.1cm}{1.1cm}{0.8cm}{0.8cm}
% {out_imgs/gt_masked_s0/bunny_v28/0003.png}}&
% \raisebox{-0.5\height}{\igr{0.12}{1.1cm}{1.1cm}{0.8cm}{0.8cm}
% {out_imgs/gt_masked_s0/bunny_v28/0017.png}}&
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
% {out_imgs/gt_masked_s0/sphere_v27/0003.png}}&
% \raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
% {out_imgs/gt_masked_s0/sphere_v27/0017.png}}
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \rotatebox[origin=c]{90}{NeuralPIL}&
% \multicolumn{2}{c}{
% \raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
% {out_imgs/test_imgs_387200_Mitsuba2_bunny_v7/0_fine_env_map.png}}}&
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \multicolumn{2}{c}{
% \raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
% {out_imgs/test_imgs_290400_Mitsuba2_sphere_v11/0_fine_env_map.png}}}
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \rotatebox[origin=c]{90}{Ours}&
% \multicolumn{2}{c}{
% \raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
% {out_imgs/v19_diffspec_bunny_masked_imgs/env_map_alpha=0.05.png}}}&
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \multicolumn{2}{c}{
% \raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
% {out_imgs/sphere_v20_diffspec_sphere_rough_L=3_a=0p05_imgs/env_map_alpha=0.05.png}}}
% \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \rotatebox[origin=c]{90}{Truth}&
% \multicolumn{2}{c}{
% \raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
% {out_imgs/gt_env_maps/20060807_wells6_hd.png}}}&
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \multicolumn{2}{c}{
% \raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
% {out_imgs/gt_env_maps/20060807_wells6_hd.png}}}
% \\
\end{tabular}
\caption{\textbf{Incident illumination estimed from the simulated globe object.} NeuralPIL fails to recover the illumination from the same multi-view images as ours. NeuralPIL provides a better reconstrution when the object geometry is known. PANDORA reconstructs the incident illumination with high fidelity while also learning the object's geometry and reflectance.}
\label{fig:sim_illum}
\end{figure}

==> figs_tex/sim_params.tex <==
\begin{figure*}
\centering
\setlength{\tabcolsep}{0pt}
\begin{tabular}{rccc@{\hskip 3pt}|@{\hskip 3pt}ccc}
 & Albedo & Roughness & Illumination
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox[origin=c]{90}{NeuralPIL}&
\raisebox{-0.5\height}{\igr{0.12}{0cm}{0cm}{0cm}{0cm}
{out_imgs/test_imgs_387200_Mitsuba2_bunny_v7/0_fine_diffuse.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0cm}{0cm}{0cm}{0cm}
{out_imgs/test_imgs_387200_Mitsuba2_bunny_v7/0_fine_roughness.png}}&
\raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/test_imgs_387200_Mitsuba2_bunny_v7/0_fine_env_map.png}}&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\raisebox{-0.5\height}{\igr{0.12}{0cm}{0cm}{0cm}{0cm}
{out_imgs/test_imgs_290400_Mitsuba2_sphere_v11/0_fine_diffuse.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0cm}{0cm}{0cm}{0cm}
{out_imgs/test_imgs_290400_Mitsuba2_sphere_v11/0_fine_roughness.png}}&
\raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/test_imgs_290400_Mitsuba2_sphere_v11/0_fine_env_map.png}}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox[origin=c]{90}{Ours}&
\raisebox{-0.5\height}{\igr{0.12}{0cm}{0cm}{0cm}{0cm}
{out_imgs/v19_diffspec_bunny_masked_imgs/pred_000_alb.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0cm}{0cm}{0cm}{0cm}
{out_imgs/v19_diffspec_bunny_masked_imgs/pred_000_rough.png}}&
\raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/v19_diffspec_bunny_masked_imgs/env_map_alpha=0.05.png}}&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\raisebox{-0.5\height}{\igr{0.12}{0cm}{0cm}{0cm}{0cm}
{out_imgs/sphere_v20_diffspec_sphere_rough_L=3_a=0p05_imgs/pred_000_alb.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0cm}{0cm}{0cm}{0cm}
{out_imgs/sphere_v20_diffspec_sphere_rough_L=3_a=0p05_imgs/pred_000_rough.png}}&
\raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sphere_v20_diffspec_sphere_rough_L=3_a=0p05_imgs/env_map_alpha=0.05.png}}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox[origin=c]{90}{Truth}&
\raisebox{-0.5\height}{\igr{0.12}{0cm}{0cm}{0cm}{0cm}
{out_imgs/v19_diffspec_bunny_masked_imgs/gt_003_alb.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0cm}{0cm}{0cm}{0cm}
{out_imgs/v19_diffspec_bunny_masked_imgs/gt_003_rough.png}}&
\raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/gt_env_maps/20060807_wells6_hd.png}}&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\raisebox{-0.5\height}{\igr{0.12}{0cm}{0cm}{0cm}{0cm}
{out_imgs/sphere_v20_diffspec_sphere_rough_L=3_a=0p05_imgs/gt_003_alb.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0cm}{0cm}{0cm}{0cm}
{out_imgs/sphere_v20_diffspec_sphere_rough_L=3_a=0p05_imgs/gt_003_rough.png}}&
\raisebox{-0.5\height}{\igr{0.24}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/gt_env_maps/20060807_wells6_hd.png}}
\\
\end{tabular}
\caption{\textbf{Radiance decomposition on scenes with smooth specular and unpolarized illumination}}
\label{fig:sim_params}
\end{figure*}

==> figs_tex/suppl_pol_vs_nopol.tex <==
\begin{figure}[ht!]
\centering
\setlength{\tabcolsep}{0pt}
% \begin{tabular}{rcccc@{\hskip 3pt}|@{\hskip 3pt}cccc}
\begin{tabular}{rcccc@{\hskip 3pt}@{\hskip 3pt}cccc}
& Mixed & Diffuse & Specular & Surface
% & Mixed & Diffuse & Specular & Surface
\\
& Radiance & Radiance & Radiance & Normals
% & Radiance & Radiance & Radiance & Normals
\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox[origin=c]{90}{Unpolarized}&
\raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_unpol/pred_000_cues_mix_s0.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_unpol/pred_000_rgb.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_unpol/pred_000_spec.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_unpol/pred_000_normal.png}}&
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox[origin=c]{90}{Ours}&
\raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_ours/pred_000_cues_mix_s0.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_ours/pred_000_rgb.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_ours/pred_000_spec.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_ours/pred_000_normal.png}}&
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rotatebox[origin=c]{90}{Truth}&
% \raisebox{-0.5\height}{\igr{0.12}{2.2cm}{2.2cm}{1.6cm}{1.6cm}
\raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_ours/gt_000_s0.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_ours/gt_000_rgb.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_ours/gt_000_specular.png}}&
\raisebox{-0.5\height}{\igr{0.12}{0.cm}{0.cm}{0.cm}{0.cm}
{out_imgs/sim_comparisons/globe_ours/gt_000_normal.png}}&
% \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\caption{\textbf{Comparison of reflectance separation and surface normals for polarized vs unpolarized inverse rendering}: We see that with polarimetric cues we are able to better estimate the surface normals while achieving similar reflectance separation.}
\label{fig:suppl_pol_vs_nopol}
\end{figure}
